Illusion of Causality in Visualized Data

Students who eat breakfast more frequently tend to have a higher grade point average. From this data, many people might confidently state that a before-school breakfast program would lead to higher grades. This is a reasoning error, because correlation does not necessarily indicate causation -- X and Y can be correlated without one directly causing the other. While this error is pervasive, its prevalence might be amplified or mitigated by the way that the data is presented to a viewer. Across three crowdsourced experiments, we examined whether how simple data relations are presented would mitigate this reasoning error. The first experiment tested examples similar to the breakfast-GPA relation, varying in the plausibility of the causal link. We asked participants to rate their level of agreement that the relation was correlated, which they rated appropriately as high. However, participants also expressed high agreement with a causal interpretation of the data. Levels of support for the causal interpretation were not equally strong across visualization types: causality ratings were highest for text descriptions and bar graphs, but weaker for scatter plots. But is this effect driven by bar graphs aggregating data into two groups or by the visual encoding type? We isolated data aggregation versus visual encoding type and examined their individual effect on perceived causality. Overall, different visualization designs afford different cognitive reasoning affordances across the same data. High levels of data aggregation by graphs tend to be associated with higher perceived causality in data. Participants perceived line and dot visual encodings as more causal than bar encodings. Our results demonstrate how some visualization designs trigger stronger causal links while choosing others can help mitigate unwarranted perceptions of causality.

==> BackupExp1_CIwith2sigfigs.tex <==
Experiment 1 Causality in Context}
Experiment 1 investigates whether visualization design influences how people interpret correlation and causation in data using the four context selected from the pilot experiment through both judgment tasks, where participants rate how much they agree with a correlation or causation statement, and generative tasks, where participants verbally interpret the information and justify their judgment task reasoning, as shown in Figure \ref{judgmentgenerativeexample}. 

\begin{figure}[htb]
 \centering
 \includegraphics[width=2.3in]{CC_Exp1_JudgmentGenerativeTask.png}
  \caption{Example of generative task (top) and judgment task (middle and bottom) in Experiment 1.}
 \label{judgmentgenerativeexample}
\end{figure}

\subsection{Participants}
Participants were recruited through the Human intelligence Task (HIT) postings on Amazon's Mechanical Turk (MTurk). We filtered for MTurk workers who are based in the United states and have an approval rate of 95\% or above. We excluded all participants who failed the attention checks, entered nonsensical answers for the free response questions or failed the graph reading comprehension checks. A omnibus power analysis based on pilot effect sizes suggested a target sample of 136 participants would give us 95\% power to detect an overall difference between visualization designs at alpha level of 0.05. We iteratively surveyed and excluded participants until we reached this sample size.

\subsection{Design}
This experiment had a $4\times4$ Graeco Latin Square design. As shown in Figure \ref{exp1_latinSquare}, each participant saw four sets of data in the four contexts chosen from the pilot experiment, presented using four visualization designs. We replicated each condition 34 times to increase the reliability in our measures. We chose three simple visualization designs commonly seen in media and education \cite{BBC2019,wp2016,tufte2001visual,knaflic2015storytelling} -- bar graphs, scatter plots and line graphs as well as a plain text, as shown in Figure \ref{teaser}. The plain text was written to parallel the bar graph, including identical information where one variable (X) was arbitrarily divided into two groups and the corresponding average value for the other variable (Y) at those two groups were specified.

\begin{figure}[htb]
 \centering
 \includegraphics[width=3.23in]{CC_Exp1_LatinSquare_Design.png}
 \caption{Graeco-Latin Square design showing the 4 conditions for Experiment 1. Each row represents a condition. Each column represents the order in which the participants saw the stimuli, with the left-most seen first and the right-most seen last.}
 \label{exp1_latinSquare}
\end{figure}

The independent variables in this experiment are the visualization designs and context plausibility. Visualization design is a categorical variable indicating the design we presented the information to the participants with, which could be bar, line, scatter plots or plain text. Context plausibility is the correlation and causation statement plausibility collected from the pilot experiment, which is a continuous variable from 0, extremely implausible, to 100, extremely plausible. Since this is a Latin Square, we recorded the order in which the participants viewed the visualizations. We also collected information on co-variables such as participant age, gender, political orientation, and level of education.

The dependent variables are correlation and causation statement agreement, which is collected from the judgment task where participants rated how much they agree with the correlation and causation statements listed in Table \ref{pilot_stories}, and the verbal conclusion characterization, which is collected from the free text responses coded by four researchers. 

\subsection{Materials}
We used MATLAB to randomly generate 100 pairs of data points from a normal distribution with a correlation of 0.6, and visualized this data set into a bar graph, a line graph, a scatter plot, as shown in Figure \ref{teaser}. To ensure all participants view the same visualization across all conditions, we relabeled the axis to fit the context without changing the underlying data set. For example, Figure \ref{bargraphs_difflabels} shows the bar graph depicted in the four context. 

\begin{figure}[htb]
 \centering
 \includegraphics[width=3.48in]{CC_Exp1_SameDesign_DiffContext.png}
 \caption{The bar graph stimulus in the four contexts.}
 \label{bargraphs_difflabels}
\end{figure}

\subsection{Procedure}
Upon accepting the HIT, participants clicked on a Qualtrics link to access the experiment. Participants completed the four task trials and finished with demographic questions. On each trial, participants viewed a visualization (bar, scatter, line or text) and answered two graph reading comprehension check questions. They then completed the generative task where they wrote several sentences explaining what they concluded from the visualization and why. This was followed by the judgment task where participants read a correlation and a causation statement (presented separately on two pages), and rated how much they agree with each on a scale from 0, which means disagree, to 100, which means agree, as shown in Figure \ref{judgmentgenerativeexample}. 













\begin{figure*}[htb]
 \centering
 \includegraphics[width=18cm]{CC_Exp1_Qual.png}
 \caption{Qualitative coding results of Experiment 1. Each bar represents the percentage participants that mentioned the indicated dimension (e.g. 3rd variable) for a certain visualization design.}
 \label{qual_exp1_exp2}
\end{figure*}

\subsection{Qualitative Results from Generative Task}
The generative task responses (where participants wrote several sentences explaining what they concluded from the visualization and why) were coded by four blind coders according to taxonomy from the pilot experiment. Each response were coded as "yes" or "no" on each of the 6 categories, as shown in the top row of Figure \ref{qual_exp1_exp2}. 

\paragraph{Correlation Conclusions} Many participants appropriately inferred correlation between depicted variables, using words and phrases such as "tend to" and "the more X the more Y" A chi-square test of independence with Bonferroni adjustment suggests that varying proportion of participants drew correlation conclusions from different visualization designs ($\chi^2$=27.84, $p$<0.001). On average, 75.7\% of the participants drew correlation conclusion from line graphs ($CI_{95\%}$=[68.65, 82.93]), 69.11\% of the participants from scatter graphs ($CI_{95\%}$=[31.35, 76.88]), 52.94\% of the participants from bar graphs ($CI_{95\%}$=[44.55, 61.32]), and 50.00\% of the participants from text ($CI_{95\%}$=[41.60, 58.40]). 
 
\paragraph{Causal Conclusions} Among the participants who generated causal conclusions from the data, in addition to participants who used causation suggestive words, we also observed responses where the participants assumed causation without using causation suggestive words such as "leads to" or "causes." Interestingly, some of these participants dismissed the visualized information as illogical because the causal relation they interpreted went against their belief or intuition. As a result, some didn't reach a conclusion from the visualization not because they were aware that correlation is not causation, but because they think the visualization is depicting a causal relation that did not make sense to them. For example, in response to the "spending and fitness" visualization, one participant suggested that the visualization did not make sense because "there is no correlation between the two," clearly mistaking correlation for causation. In this case, the response was coded for both "causation" and "no conclusion."
\vspace{1.5pt}
\noindent\textit{"The data tries to suggest that sending more on sporting events somehow increases a person's physical fitness. That makes no sense. I believe that people who have a deep appreciation for athletics also have an appreciation for fitness in general, but being a fan does not make someone fit."}

There are also two participants who mentioned "experiments" in their responses, even though we specifically noted that the visualizations are generated from survey data. It is possible that some people are more likely to make causal conclusions under some visualization design than others because they associate that specific design with controlled experiments, from which causal conclusions can be validly drawn. 

We found several common characteristics among participants who did not assume causal relations. They questioned the directionality and predispositions, or mentioned third variables at play. For example, in the "breakfast and GPA" context, participants who did not assume causation questioned whether it is people who ate breakfast more were more likely to get good grades, or that people who were more likely to get good grades were more organized, and thus more likely to get up early and eat breakfast. 

A chi-square test of independence revealed an overall effect of visualization design on whether people drew causal conclusions ($\chi^{2}$=21.77, $p$<0.0001). As shown in the causation column in Figure \ref{qual_exp1_exp2}, on average, 38.97\% of the participants drew causal conclusion from text graphs ($CI_{95\%}$=[30.77, 47.17]), 33.82\% of the participants from bar graphs ($CI_{95\%}$=[25.87, 41.77]), 20.59\% of the participants from scatter plots ($CI_{95\%}$=[13.79, 27.38]), and 18.38\% of the participants from line graphs ($CI_{95\%}$=[11.87, 24.89]). 

\paragraph{Third Variables?} How might visualization design influence whether people think of third variables or not when drawing conclusions from visualizations? 

We observed participants justifying both correlation and causation connecting a third variable to the two visualized. For example, in the "internet and homicide" context, one participant speculated that "using Internet Explorer \textit{causes} homicide rates to rise because using Internet Explore creates anger, and anger leads to homicides." Anger is not visualized on the graph, therefore it is a third variable. 

A chi-square test of independence revealed that there is no relation between visualization design and mentioning of third variables ($\chi^{2}$=2.03, $p$=0.57), suggesting no particular visualization design makes people more or less likely to think of third variables, as shown in the $3^{rd}$ variable column in Figure \ref{qual_exp1_exp2}. On average, 30.88\% of the participants mentioned third variables in scatter plots ($CI_{95\%}$=[23.12, 38.65]), 30.88\% of the participants in text ($CI_{95\%}$=[23.12, 38.65]), 30.15\% of the participants in line graphs ($CI_{95\%}$=[22.43, 37.86]), and 24.26\% of the participants in bar graphs ($CI_{95\%}$=[17.06, 31.47]). 

\paragraph{Grouping in Response} We observed an overall effect of visualization design on the amount of group-wise comparisons made ($\chi^{2}$=15.57, $p$<0.001). Raters coded responses as group-wise comparisons when the participant described the visualized data in two groups by one dimension and compared the 2 grouped values in the other dimension, such as 
\vspace{1.5pt}
\noindent\textit{"The students who ate less than four breakfasts a week had a lower GPA than those who ate more than four breakfasts a week."}

On average, 27.94\% of the participants made group-wise comparisons of variables in bar graphs ($CI_{95\%}$=[20.40, 35.48]), 16.18\% of the participants in text ($CI_{95\%}$=[9.99, 22.37]), 16.18\% of the participants in scatter plots ($CI_{95\%}$=[9.99, 22.37]), and 9.56\% of the participants in line graphs ($CI_{95\%}$=[4.62, 14.50]). 

\paragraph{Direct Observations} While no visualization elicited more direct observations than others $\chi^{2}$=5.09, $p$=0.17), we observed several direct, number-specific comparisons instead of global pattern or trend observations across all designs. For example, when viewing a bar visualization on "breakfast and GPA," one participant concluded the following information. 
\vspace{1.5pt}
\noindent\textit{"On average, students who eat less than 4 breakfasts per week has average GPA around 3.0."}

On average, 11.03\% of the participants made direct observations in bar graphs ($CI_{95\%}$=[5.76, 16.29]), 6.61\% of the participants in scatter plots ($CI_{95\%}$=[2.44, 10.80]), 5.88\% of the participants in text ($CI_{95\%}$=[1.93, 9.83]), and 4.41\% of the participants in line graphs ($CI_{95\%}$=[0.96, 7.86]). 

\paragraph{No Conclusions} No visualization elicited more non conclusions than others ($\chi^{2}$=2.57, $p$=0.46). On average, 11.03\% of the participants drew no conclusion in text ($CI_{95\%}$=[5.76, 16.29]), 8.09\% of the participants in bar graphs ($CI_{95\%}$=[3.51, 12.69]), 7.35\% of the participants in line graphs ($CI_{95\%}$=[2.97, 11.74]), and 5.88\% of the participants in scatter plots ($CI_{95\%}$=[1.93, 9.84]). 

We observed two types of no conclusion responses, one where participants inferred causality from the visual but decided to draw no conclusion because it went against their intuition, and the other where participants made a conscious decision not to. This could be a result of them choosing to be skeptical about the completeness of the information or being aware of "correlation is not causation." For example, in response to the "internet and homicide" context, one participant wrote --
\vspace{1.5pt}
\noindent\textit{"I am not sure I can conclude anything…the use of Internet Explorer may have declined at the same time the murder rate declined with no connection except coincidence."}

In general, many people drew from their personal experience, knowledge or history to make sense of the visualized information. Congruent with prior research, most participants' first intuition is to justify a potential relation between the variables visualized, despite the plausibility of the causal link \cite{ibrahim2016using, kahneman2011thinking}. Few stopped and thought of "counter examples," questioned the validity of the data, or showed clear signs of understanding that correlation is not causation. 

Some participants used "template" words or phrases, such as "correlation is not causation" or "Y tend to increase with varying levels of X" to frame their conclusions. For example, one participant made the following conclusion in the "internet and homicide" scenario.
\vspace{1.5pt}
\noindent\textit{"The graph shows that in cities with more people using Internet Explorer, there tend to be many more homicides. While the results are pretty clear, I think "correlation is not causation" should be applied here. I'm not a scientist, but I don't think the two variables are really related in any meaningful way."}

It is also apparent when a participant only memorized the phrase "correlation is not causation" without truly understanding the concept. They read correlation from the data, and assumed the data to be telling a causal story as they equated correlation and causation in their head. But because they were superficially aware that "correlation is not causation," they dismissed the \textit{correlation} in data despite the observable correlation in data. This is as dangerous as n{\"a}ively assuming causation in data because the viewer, while dismissing all correlational evidences in data, may fail to see hidden information such as third-variable links. For example, this participant was clearly aware of the phrase "correlation is not causation," but instead of critically thinking through third variables or other possibilities, quickly dismissed the data and the apparent correlation. \newline
\vspace{1.5pt}
\noindent\textit{"With only this information I cannot conclude anything since I do not see any correlation. In my opinion these two variables are uncorrelated..."}

Furthermore, participants all interpreted the visualization assuming the X -> Y directionality, such as "as X increases Y increases." For people who made causal conclusions, all of them described the x-axis variable as the cause and the y-axis variable as the effect. This suggests that there may exist a conventional interpretation of causality in data for the x-axis variable to be seen as the cause and the y-axis variable to be seen as the causee. 

















\subsection{Causation Judgment Results}
We used a mixed-effect linear model to fit the causation ratings, which was how much each participant agreed with the causation statements, under the four visualization designs (bar, scatter, line and text). For fixed effects, we used visualization design, causation statement plausibility, trial order and demographic information (age, gender, education and political orientation) as predictors. Because perceived causality could be both visualization design dependent and context dependent \cite{pandey2014persuasive}, we also considered an interaction between visualization design and causation statement plausibility. We used a random intercept term accounting for individual differences as random effects.

The regression model indicated a large effect of causation statement plausibility (context), $\chi^2$=162.70, $\eta_{partial}^{2}$=0.274,$p$<0.001, a small effect of visualization design ($\chi^2$=11.65,$\eta_{partial}^{2}$=0.026,$p$<0.01), and negligible interaction effect between causation statement plausibility (context) and visualization design ($\chi^2$=0.97,$\eta_{partial}^{2}$=0.002,$p$=0.81). Referencing Figure \ref{quant_exp1_exp2}, participants rated bar graphs to be the most causal ($M$=76.59, $CI_{95\%}$=[71.51, 81.76]) and text the second most causal ($M$=71.26, $CI_{95\%}$=[65.30, 77.23]). This largely agreed with the results from the generative tasks where participants also made causal interpretations and the most group-wise comparisons in bar graphs and text. Given the similarity between bar graph and text, which was written to contain identical information as the bar graph (grouping the data into 2 groups), we suspect that perceived causality differed between visualization designs because information was organized and presented differently among them. 

Line graphs and scatter plots, unlike bar graphs and text, did not group variables together. Participants rated line graphs ($M$=68.43, $CI_{95\%}$=[62.52, 74.35]) and scatter plots ($M$=67.29, $CI_{95\%}$=[61.52, 73.07]) the least causal, which were the two designs with the most correlation interpretation in the generative task. This suggests that the effect of visualization design on perceived causality could be driven by data aggregation and visual encoding marks.

There is negligible effect of the order the visualizations were presented ($\chi^2$=0.11,$\eta_{partial}^{2}$=0.002, $p$=0.74), which means perceived causation does not depend on what was presented to them previously nor was there a learning effect. For individual differences, there is negligible effect of age ($\chi^2$=0.49,$\eta_{partial}^{2}$=0.002, $p$=0.48) and political orientation ($\chi^2$=0.73,$\eta_{partial}^{2}$=0.001, $p$=0.39), but a small effect of gender ($\chi^2$=4.23,$\eta_{partial}^{2}$=0.007,$p$=0.040), such that male participants gave higher causation ratings, and education ($\chi^2$=0.4.53, $\eta_{partial}^{2}$=0.011,$p$=0.033), such that participants who were more educated gave lower causation ratings.

\begin{figure}[htb]
 \centering
 \includegraphics[width=8.8cm]{CC_Exp1_Quant.png}
 \caption{Quantitative results from Experiment 1. Solid lines represent causation and dotted lines represent correlation.}
 \label{quant_exp1_exp2}
\end{figure}

\subsection{Correlation Judgment Results}
We used a similar mixed-effect linear model to predict how much each participant agreed with the correlation statements. We kept all predictors the same with the exception of swapping the causation statement plausibility for the correlation statement plausibility. Only correlation statement plausibility had a sizable effect predicting perceived correlations ($\chi^2$=71.02,$\eta_{partial}^{2}$=0.141,$p$<0.001), there was negligible effect of visualization design ($\chi^2$=1.98,$\eta_{partial}^{2}$=0.005,$p$=0.58), a small interaction between the two ($\chi^2$=6.15,$\eta_{partial}^{2}$=0.012,$p$=0.10), a tiny effect of education ($\chi^2$=2.99,$\eta_{partial}^{2}$=0.007,$p$=0.08), negligible effect of order, age and gender, details included in the supplementary. We can see this from the relatively identical correlation confidence intervals in Figure \ref{quant_exp1_exp2}. This suggests visualization design does not significantly influence people's judgment of correlation from data, at least when participants were given a concrete context.

\subsection{Discussion} 
In general, the quantitative and qualitative results told similar stories of how, with concrete context, people perceived the most causality in bar and text graphs, and less from line and scatter graphs. Context also had a large effect on perceived causality, but the effect of visualization design on perceived causality was not context dependent. We took away the concrete context in subsequent experiments to further examine \textit{how} visualization designs influence perceived causality. 




==> No-Exp2_4AbstractExamples.tex <==
\section{Experiment 2 Causality without context}
Although the visualization context did not influence the effect of visualization design on perceived causality, itself had a large effect on perceived causality. Experiment 2 stripped context away from the visualizations to 

\subsection{Methods}
Experiment 2 used four visualization design identical to that in Experiment 1. Instead of presenting the data in four scenarios with varying plausibility, we stripped the variable names (e.g., "GPA") and replaced with abstract variable labels (e.g., "X","Y"). 

We used a within-subject design where every participant viewed all four visualizations (bar, scatter, line or text) in random order. For each visualization, they completed the same graph reading comprehension check questions, conclusion generating tasks and correlation and causation statement agreement judgment tasks as in Experiment 1. We collected data on the same independent variables and dependent variables as Experiment 1 and analyzed them following the methods in Experiment 1.

Participants were recruited through the Human intelligence Task (HIT) with the same preliminary quality check and exclusion criteria. A omnibus power analysis based on pilot effect sizes suggested a target sample of 31 participants would give us 95\% power to detect an overall difference between visualization designs at alpha level of 0.05.













\subsection{Qualitative Coding Results of the Generative Tasks}
Following the same analytic methods as that in Experiment 1, we found that the effect of visualization design persists even when we strip context from the visualizations, as shown in the bottom row of Figure \ref{qual_exp1_exp2}.

\paragraph{Correlation Conclusions} Replicating the findings of Experiment 1, the amount of people who drew correlation conclusions from figures differed between visualization designs ($\chi^{2}$=17.80, $p$<0.001). 

On average, 27.94\% of the participants made group-wise comparisons of variables in bar graphs ($CI_{95\%}$=[20.40, 35.48]), 16.18\% of the participants in text ($CI_{95\%}$=[9.99, 22.37]), 16.18\% of the participants in scatter plots ($CI_{95\%}$=[9.99, 22.37]), and 9.56\% of the participants in line graphs ($CI_{95\%}$=[4.62, 14.50]). 

Here is one example of drawing correlation conclusions
\vspace{1.5pt}

\noindent\textit{"As X increases, do does Y. I decided this becasue when X moves from low to high there is a large change in Y as well, also going from lower to higher.}

\paragraph{Causal Conclusions}


Here is one example of drawing correlation conclusions
\vspace{1.5pt}

\noindent\textit{"As X increases, do does Y. I decided this becasue when X moves from low to high there is a large change in Y as well, also going from lower to higher.}





\paragraph{Third Variable} Interestingly, no one mentioned third variables in Experiment 2. We speculate this to be a product of context abstraction in data. 

\paragraph{Grouping in Response} Furthermore, people made direct observation where they described the information by "grouping" the variables. Following the intuition of the Northwestern instructor at Kellogg Business School, as shown in  \textcolor{CX}{Figure}, they did this much more often in bar graphs than in other visualization designs (\begin{math}\chi^{2}=21.99\end{math}, p<0.001). 

\paragraph{Direct Observations} As shown in Figure \ref{qual_exp1_exp2}, people became more likely to make direct observations because of this abstraction when there is no context. Chi-square analysis revealed that there is a significant relation between visualization design and the conclusions participants generated,  \begin{math}\chi^{2}=22.56\end{math}, p=0.0073. 

\paragraph{No Conclusions}























\subsection{Causation Judgment Results}
participants rated text the most causal ($M$=96.65, $CI_{95\%}$=[93.67, 99.62])

We used a mixed-effect linear model to fit causation agreement for the four visualization designs (bar,  scatter,  line and text), adding co-variables including age, gender, education and political orientation as fixed effects. We used a random intercept term to account for individual differences as random effects. As shown in the regression model summary in Table 5, there is a significant effect of visualization design (p<0.001) and, as shown in \textcolor{CX}{Figure 10}, age (p=0.034) on how much participants agreed with the causation statement.

Post-hoc analysis revealed that among the visualization designs, as shown in \textcolor{CX}{Figure 11}, adjusted for multiple comparisons, people agreed with the causation statement the most in plain text, line graphs, bar graphs, and least in scatter plot. This agrees with findings in Experiment 1 suggesting that plain text leads to problematic causal interpretations that can be slightly alleviated by visualizations, especially scatter plots. 

\subsection{Correlation Judgment Results}

Upon close examination of correlation statement agreement in Experiment 2, using again a mixed-effect regression model using text design as reference, as shown in \textcolor{CX}{Figure} and \textcolor{CX}{Figure}, we find that in this iteration, education and political orientation, in addition to visualization design, can significantly predict correlation agreement. 

We can plot the correlation and causation agreement in Experiment 2 on the same graph, and notice how, as shown in \textcolor{CX}{Figure}, once we remove the context, participants essentially interpret correlation to be identical to causation. While the effect of visualization design seem to persist (p<0.001), there is no significant main effect of correlation and causation statement (p=0.65), nor a significant interaction of correlation and causation statement on visualization design (p=0.954).


\subsection{Discussions}

Experiment 2 supplements the findings in Experiment 1, suggesting that without context, text, bars, lines and scatter points on a visualization triggers fundamentally different intuitive reactions. Since we referenced the bar graphs to generate the text, it makes sense that both bar graphs and text elicits similar levels of causal thinking across experiment. This extends theories on graph schema to further include shapes in visualizations (e.g., bars and lines) to afford different reasoning intuitions. We see that visualizing the information overall reduces the likelihood of information viewers agreeing with or drawing problematic causal conclusions. And among visualizations, scatter plots and line graphs invites the least amount of causal assumptions. 

\jessica{in skimming this section to try to see what experiment 2 adds, I'm left unsure from the above paragraph. Are things consistent with exp 1 or not? If they are, then I don't know that we shoudl be reporting exp 2, as it only seems to question the validity of exp 1 . If it conflicts, that's even more problematic}

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> StatsDeposit.tex <==
Experiment 3a


trend - line == 0           -10.8909     3.2575  -3.343 0.017386 * 
trend - 7bar == 0            -9.6727     3.2575  -2.969 0.062673 . 
7bar - 2bar == 0             12.6000     3.2575   3.868 0.002305 ** 
trend - group == 0            9.1818     3.2575   2.819 0.101278  

line - 7bar == 0              1.2182     3.2575   0.374 1.000000    
2scatter - 2bar == 0         -0.8182     3.2575  -0.251 1.000000    
group - 2bar == 0            -6.2545     3.2575  -1.920 1.000000  
trend - 2bar == 0             2.9273     3.2575   0.899 1.000000  
group - 2scatter == 0        -5.4364     3.2575  -1.669 1.000000   
trend - 2scatter == 0         3.7455     3.2575   1.150 1.000000   

line - 2bar == 0             13.8182     3.2575   4.242 0.000465 ***
manyscatter - 2bar == 0     -14.9091     3.2575  -4.577 9.92e-05 ***
7bar - 2scatter == 0         13.4182     3.2575   4.119 0.000799 ***
line - 2scatter == 0         14.6364     3.2575   4.493 0.000147 ***
manyscatter - 2scatter == 0 -14.0909     3.2575  -4.326 0.000319 ***
group - 7bar == 0           -18.8545     3.2575  -5.788 1.50e-07 ***
manyscatter - 7bar == 0     -27.5091     3.2575  -8.445  < 2e-16 ***
line - group == 0            20.0727     3.2575   6.162 1.51e-08 ***
manyscatter - group == 0     -8.6545     3.2575  -2.657 0.165673    
manyscatter - line == 0     -28.7273     3.2575  -8.819  < 2e-16 ***
trend - manyscatter == 0     17.8364     3.2575   5.475 9.17e-07 ***

----


line - 7bar == 0               1.145      3.347   0.342 1.000000 
trend - line == 0             -4.909      3.347  -1.467 1.000000 
trend - 7bar == 0             -3.764      3.347  -1.124 1.000000 
trend - 2bar == 0              6.709      3.347   2.005 0.945330  
 
2scatter - 2bar == 0          -5.945      3.347  -1.776 1.000000  
group - 2bar == 0             -4.473      3.347  -1.336 1.000000  
group - 2scatter == 0          1.473      3.347   0.440 1.000000 
manyscatter - 2scatter == 0   -4.309      3.347  -1.287 1.000000    
manyscatter - group == 0      -5.782      3.347  -1.727 1.000000    

7bar - 2bar == 0              10.473      3.347   3.129 0.036836 *  
line - 2bar == 0              11.618      3.347   3.471 0.010880 *  
manyscatter - 2bar == 0      -10.255      3.347  -3.064 0.045894 *  
7bar - 2scatter == 0          16.418      3.347   4.905 1.96e-05 ***
line - 2scatter == 0          17.564      3.347   5.248 3.24e-06 ***
trend - 2scatter == 0         12.655      3.347   3.781 0.003282 **
group - 7bar == 0            -14.945      3.347  -4.465 0.000168 ***
manyscatter - 7bar == 0      -20.727      3.347  -6.193 1.24e-08 ***
  
line - group == 0             16.091      3.347   4.808 3.21e-05 ***
trend - group == 0            11.182      3.347   3.341 0.017540 *  
manyscatter - line == 0      -21.873      3.347  -6.535 1.34e-09 ***
trend - manyscatter == 0      16.964      3.347   5.068 8.43e-06 ***


further shows that causality perception could 

Bar graphs and the group-flavoured text description aggregated data into two groups, while line graphs illustrated continuous data, and scatter plot illustrated continuous data in a discretized way, depicting detailed information for each subject. 

whether they aggregated data into two groups  

Experiment 2 compared perceived causality in designs that aggregate data into two groups (in bar graphs and group-flavoured text descriptions) 

line graphs, scatter plots with many scatter points, bar graphs with 2 bars, and 

- visualization designs afford different cognitive reasoning 
- we see bar graph = perceived more causal, scatter plot = perceived less causal 
- but that's an artifact of how/what information is presented rather than the actual visuals of bars, lines and dots 
- once we discretize everything, bars are perceived to be less causal
- (speculation) in addition to aggregating or discretizing data, people have schemas associated with bars, lines and dots



\subsubsection{Interaction between Correlation and Causation}

We can further model how visualization design interact with how people judge correlation and causation in data. As shown in \textcolor{CX}{Figure}, there is a main effect of correlation (M=99.23) and causation (M=71.27) statement agreement ratings (p<0.001), which suggests that on average, people are able to distinguish correlation and causation to an extent. They agree more strongly with correct correlation statements describing visualized variable relations, and less strongly with causation statements that incorrectly infer causal relations. 
There is no significant main effect of visualization designs (p=0.12), but post-hoc comparisons, with a Bonferroni adjustment, reveals that there is a trending effect of visualization design in overall agreement of correlation and causation statements between bar graphs (M=88.29) and scatter plot (M=77.39, p=0.059). There is also no significant interaction of visualization designs and whether the statement is a correlation one or a causation one (p=0.48). This is expected as the effect of whether the statement is a correlation statement or a causation one is very large  (\begin{math}R_{partial}^{2}=0.93\end{math}, whereas the effect size of visualization is relatively small (\begin{math}R_{partial}^{2}=0.048\end{math}). 

This suggests that in judgment tasks where people read correlation and causation statements, because the language of the statements itself has a strong effect triggering people to associate it with correlation or causation, the effect of visualization, although present, becomes relatively weak and negligible. However, despite the small effect, visualizing information using scatter plot can marginally make people less likely to agree with fallacious causal statements than using bar graphs. 


On the other hand, some participants thought of third variables and dismissed potential causal relations as spurious correlations associated with the third variables. For example, when viewing the visualization on "sports and spending," one participant speculated that "people who are physically fit likely do sports themselves. This means they are more likely to attend games to watch those sports." In this scenario, the participant acknowledge a correlation between physical fitness and money spent on sporting events. They justified this correlation using third variable - enjoyment doing sports, without assuming causation. 



People also made the least amount of group-wise comparison in line graphs ($p$<0.01), as shown in Figure \ref{qual_exp1_exp2}.

\begin{figure*}[htb]
 \centering
 \includegraphics[width=18cm]{CC_Exp3ab_Exp4_Consolidated.png}
 \caption{Consolidated results from Experiment 3a, 3b and 4. Bars indicate average causation ratings. Benchmark lines indicates average correlation ratings.Top left is results from Experiment 3a, top right from Experiment 3b, and bottom left from Experiment 4.}
 \label{fig:Exp3ab_Exp4_consolidated}
\end{figure*}



----
Experiment 1 and 2
2 ways bars adn scatter differ
bars aggregate into fewer bins,
which of those drove?
2 by 3
aggregation level and visualization type 

main effect of aggregation level
main effect of visual encoding type, 

changing scatter to a dot plot, 

explicitly say it's aggregated.

2 and 16 

\section{Experiment 2 Aggregation levels}
Experiment 1 found that people perceived high causality from bar graphs and text, and low causality from scatter plots. But is this driven by the visual encoding marks (e.g., rectangular bars versus circular points versus lines), or by the amount of aggregation in data? For example, the bar graph we showed aggregated the data into 2 groups while the scatter plot did not aggregate any data, showing each data points individually. While we suspect both factors to influence perceived causality, we need to empirically test them. Experiment 3 test the effect of the amount of aggregation in data on perceived causality, and whether the visual encoding marks interacts with this effect by comparing bar graphs, line graphs and scatter plots.

\begin{figure}[htb]
 \centering
 \includegraphics[width=8cm]{CC_Exp3_Design.png}
 \caption{Aggregation levels tested in Experiment 3 for bar, line and dot type encoding marks.}
 \label{exp3DesignAggregationLevel}
\end{figure}

\subsection{Design}
Because visualization context did not influence the effect of visualization design on perceived causality, we stripped context away from the visualizations in this experiment. Instead of presenting the data in four scenarios with varying plausibility, we stripped the variable names (e.g., "GPA") and replaced with abstract variable labels (e.g., "X","Y"). 

We operationalized the amount of aggregation as the number of bins the data is sorted in. The bar graph used in Experiment 1 and 2 aggregated the data into 2 bins. We created bar graphs that aggregated the data into 8 bins and 16 bins. Although binning scattered dots and lines are rarely done, we created dot plots and line graphs using the same binned data in the bar graphs, but replacing the rectangular bars with circles and lines, as shown in Figure \ref{exp3DesignAggregationLevel}. Here, bar graphs depict comparisons of data between 2 groups, between 8 groups, or between 16 groups, which fits regular conventions of graphic communication using bar graphs\cite{zacks1999bars}. However, conventional scatter plots illustrate with each dot an individual data value \cite{sarikayascatter2018} and conventional line graphs illustrate trends generated by consolidating all data points \cite{levy1996gratuitous}, different from the line graphs and dot plots shown in this experiment, which depicts binned data, aggregated into 2, 8 or 16 groups. To ensure the participants in this experiment understand, we created an instruction with examples for participants to read through, as shown in Figure \ref{exp3instruct}.

\begin{figure}[htb]
 \centering
 \includegraphics[width=8cm]{CC_Exp3_Instructions.png}
 \caption{Snapshots of instructions with examples given to participants prior to starting Experiment 3.}
 \label{exp3instruct}
\end{figure}

During the experiment, the participants were explicitly told that the visualized data were generated by summarizing and binning data as they viewed the visualizations, as shown in the left figure in Figure \ref{exp3exp4snapshotofexp}. They completed the judgment task rating how much they agreed with correlation and causation statements, similar to Experiment 1, but we excluded the generative task here because the variables were abstract variables. We asked each participant 6 graph comprehension questions and excluded participants who did not understand the data aggregation in the experiment. The full experiment and data are in the supplementary materials.

\begin{figure}[htb]
 \centering
 \includegraphics[width=8cm]{CC_Exp3Exp4_ExperimentSnapshot.png}
 \caption{Snap shots from Experiment 3 (left) and Experiment 4 (right).}
 \label{exp3exp4snapshotofexp}
\end{figure}

The independent variables in this experiments are visual encoding marks, which can be rectangular bars, lines or dots, and aggregation level, which can be 2, 8 or 16. The dependent variables are correlation ratings and causation ratings, similar to experiment 1. We used a $3\times3$ Graeco Latin Square design crossing visualization design and aggregation groups, similar to that in Experiment 1, which crossed visualization design and context. Each participant saw three visualizations --- line graph, dot plot and bar graphs, one of which aggregated into 2 groups, one into 8 groups and other other 16 groups. 129 participants were recruited in this experiment, 43 in each condition of the Latin Square.



















\begin{figure}[htb]
 \centering
 \includegraphics[width=8.7cm]{CC_Exp3_Quant_EncodingAggregation.png}
 \caption{Main effect of visual encoding types and aggregation levels in Experiment 3.}
 \label{exp3_quant_maineffects}
\end{figure}

\subsection{Causation Judgment Results}
We used a similar mixed-effect linear model from Experiment 1 to fit the causation ratings with fixed effects of visual encoding marks, aggregation level, an interaction between encoding marks and aggregation level, trial order and demographic information (age, gender, education and political orientation), and a random intercept term accounting for individual differences as random effects. 

The regression model indicated a small main effect of visual encoding marks ($\eta_{partial}^{2}$=0.020,$p$=0.050), such that aggregated dot plots had the highest causality ratings ($M$=79.38, $CI_{95\%}$=[75.67, 83.09]), followed by line encodings ($M$=77.78, $CI_{95\%}$=[73.29, 82.26]), and rectangular bar encodings had the lowest causality ratings ($M$=74.32, $CI_{95\%}$=[69.73, 78.90]), as shown in the top row in Figure \ref{exp3_quant_maineffects}

There is large main effect of aggregation level ($\eta_{partial}^{2}$=0.29,$p$<0.001), such that visualizations with the more data aggregation were perceived as more causal. Visualizations with aggregation level 2, the most aggregation which binned data into 2 groups, had the highest average causality ratings ($M$=84.76, $CI_{95\%}$=[81.00, 88.55]), followed by visualizations with aggregation level 8 ($M$=82.95, $CI_{95\%}$=[79.16, 86.75], and visualization with the least aggregation, which binned data into 16 groups, had the lowest average causality ratings ($M$=63.74, $CI_{95\%}$=[59.46, 68.03]), as shown in the bottom row in Figure \ref{exp3_quant_maineffects}.



\begin{figure}[htb]
 \centering
 \includegraphics[width=8.7cm]{CC_Exp3_Quant.png}
 \caption{Quantitative results from Experiment 3.}
 \label{exp3_quant}
\end{figure}

There is a medium interaction effect between visual encoding marks and aggregation level ($\eta_{partial}^{2}$=0.089,$p$<0.01) on perceived causality.
For dot encodings, perceived causality did not differ significantly between aggregation level 2 ($M$=87.19, $CI_{95\%}$=82.54, 91.84]), aggregation level 8 ($M$=74.53, $CI_{95\%}$=[66.51,82.56]) and aggregation level 16 ($M$=76.42, $CI_{95\%}$=[70.42,82.41]). For line encodings, perceived causality significantly decreased as the number bins increased, such that aggregation level 2 ($M$=94.37, $CI_{95\%}$=[91.76,96.98]) was perceived the most causal, followed by aggregation level 8 ($M$=84.91, $CI_{95\%}$=[78.55,91.26]), and aggregation level 16 was perceived the least causal ($M$=54.05, $CI_{95\%}$=[46.43,61.67]). For bar encodings, aggregation level 8 was the perceived the most causal ($M$=89.42, $CI_{95\%}$=[84.85,93.98]), followed by aggregation level 2 ($M$=72.77, $CI_{95\%}$=[63.62, 81.92]), and aggregation level 16 the least causal ($M$=60.77, $CI_{95\%}$=[53.33, 68.20]).

There is negligible effect of the order the visualizations were presented ($\eta_{partial}^{2}$=0.002, $p$=0.71). For individual differences, there is negligible effect of age ($\eta_{partial}^{2}$=0.001, $p$=0.70), political orientation ($\eta_{partial}^{2}$=0.001, $p$=0.95) and gender ($\eta_{partial}^{2}$=0.002,$p$=0.70), but a small effect of education ($\eta_{partial}^{2}$=0.009, $p$=0.99). 










\subsection{Correlation Judgment Results}
We used the same mixed-effect linear model to fit the correlation ratings. The model indicated a small main effect of visual encoding marks ($\eta_{partial}^{2}$=0.03,$p$<0.01), such that aggregated dot plots had the highest correlation ratings ($M$=87.67, $CI_{95\%}$=[85.23, 90.11]), followed by line encodings ($M$=84.69, $CI_{95\%}$=[81.06, 88.32]), and rectangular bar encodings had the lowest ratings ($M$=82.10, $CI_{95\%}$=[78.17, 86.03]).


There is large main effect of aggregation level ($\eta_{partial}^{2}$=0.40,$p$<0.001), such that visualizations with the more data aggregation were perceived as more correlational. Visualizations with aggregation level 2, the most aggregation which binned data into 2 groups, had the highest average correlation ratings ($M$=92.32, $CI_{95\%}$=[89.85, 94.79]), followed by visualizations with aggregation level 8 ($M$=92.31, $CI_{95\%}$=[90.39, 94.25], and visualization with the least aggregation, which binned data into 16 groups, had the lowest average ratings ($M$=69.82, $CI_{95\%}$=[65.96, 73.68]).

There is a medium interaction effect between visual encoding marks and aggregation level ($\eta_{partial}^{2}$=0.088,$p$<0.001) on perceived correlation. 
For dot encodings, perceived correlation did not differ significantly between aggregation level 2 ($M$=91.77, $CI_{95\%}$=87.88, 95.66]), aggregation level 8 ($M$=88.28, $CI_{95\%}$=[83.49,93.06]) and aggregation level 16 ($M$=82.95, $CI_{95\%}$=[79.12,86.79]). For line encodings, perceived causality significantly decreased as the number bins increased, such that aggregation level 2 ($M$=96.42, $CI_{95\%}$=94.49,98.35]) was perceived the most causal, followed by aggregation level 8 ($M$=93.37, $CI_{95\%}$=[91.03,95.72]), and aggregation level 16 was perceived the least causal ($M$=64.28, $CI_{95\%}$=[56.88,71.68]). For bar encodings, aggregation level 8 was the perceived the most causal ($M$=95.30, $CI_{95\%}$=[93.18,97.43]), followed by aggregation level 2 ($M$=88.77, $CI_{95\%}$=[82.74, 94.80]), and aggregation level 16 the least causal ($M$=62.23, $CI_{95\%}$=[55.39, 69.07]).

There is a small effect of the order the visualizations were presented ($\eta_{partial}^{2}$=0.022, $p$=0.001), indicating a learning effect, which is reasonable given the novelty of the visualization designs. For individual differences, there is negligible effect of age ($\eta_{partial}^{2}$=0.003, $p$=0.40), and gender ($\eta_{partial}^{2}$=0.002,$p$=0.92), but a small effect of political orientation ($\eta_{partial}^{2}$=0.013, $p$=0.17) and education ($\eta_{partial}^{2}$=0.019, $p$=0.84). 



\subsection{Discussion}
The results of Experiment 3 suggests that 

the amount of aggregation has an effect on perceived causality. 
Doesn't depend on visual encoding mark.
However, since scatter plots and line graphs don't usually bin data the way bar graphs does it, it's unfair to test them in these strange set-ups.

We created Experiment 4, where there is no aggregation, to test the effect of visual encoding marks.


The present project investigated how people perceive causality from different visualization designs. We compared across familiar visualizations, such as simple bar graphs, line graphs and scatter plots as those commonly used in education and media \cite{knaflic2015storytelling}, as well as unfamiliar visualizations that discretized values to specifically test the effect of visual mark encoding types. We found the discretized visuals to reduce perceived causality, but how much of this reduction can be attributed to the unfamiliarity of the design? While we provided detailed explanations teaching participants how to read the discretized visualizations in Experiment 4 and excluded participants who failed the comprehension tests, further experimentation is necessary to isolate the effect of familiarity of visualization. 

We tested four concrete context in Experiment 1, and used abstract variables in the subsequent experiments. Comparing the qualitative and quantitative results between the two, we found similar results for perceived causation but significant differences between how correlation is interpreted from visualizations, as participants could no longer rely on their intuition or experience when judging correlation in abstract contexts. Further iterations of this experiment could examine how people perceive correlation and causation in concrete context depicting unfamiliar examples to which intuition or past experiences couldn't be easily applied. 

All the visualization designs utilized the same data set in our experiments, which means the correlation depicted was always an upward trend. We purposefully chose this positive correlation to avoid common reasoning errors such as misinterpreting negative correlations to be smaller correlations  \cite{huff1993lie}. The goal of this experiment is to investigate whether visualization design can elicit varying degrees of perceived causality in data, but further research should investigate whether the strength and direction of the correlation also have an impact. 

In our judgment tasks where participants rated how much they agree with correlation or causation statement describing the data, participants could have applied judging criteria varying in degree of leniency. Some could have rated "agree" if the statement was plausible, while others only rated "agree" if they thought the statement was correct. Future researchers can further investigate the how perceived plausibility and correctness of correlation and causation statements interact and vary with visualization designs.

Our qualitative characterizing of verbal responses may be imperfect. In this experiment, after consulting with expert instructor of research methods at Northwestern University, we identified six dimension to evaluate the content of the free response question. We encountered many instances of ambiguous language, such as "there is sort sort of relationship between A and B," which made it difficult for raters to decide whether the participants meant a correlation or a causal relation. We also found that some participants used template phrases or words, such as "correlation is not causation" and "A is correlated with B" to describe relations in data, but we lack further information to evaluate whether they actually read a causal relation from the data or not. 

Lastly, we conducted omnibus power analysis for all experiments. While we observed several insignificant differences in our pair-wise comparisons of the effect of visualization designs on perceived causation, such as the discrete line and discrete scatter point conditions in Experiment 4, it did not necessarily mean people perceive the same degree of causality in them. Further iterations of this experiment, if more resources are available, can increase the sample size and further test for any differences. 




 

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> oldExp3_7AbstractExamplesab.tex <==
\begin{figure*}[htb]
 \centering
 \includegraphics[width=18cm]{CC_Exp3ab_Exp4_Consolidated.png}
 \caption{Consolidated results from Experiment 3a, 3b and 4. Bars indicate average causation ratings. Benchmark lines indicates average correlation ratings.Top left is results from Experiment 3a, top right from Experiment 3b, and bottom left from Experiment 4.}
 \label{fig:Exp3ab_Exp4_consolidated}
\end{figure*}


\subsection{Experiment 3}
\textcolor{red}{for cindy: need to change scatter-50 points to 100 points}
In experiment 2, in addition to graph choice, the 4 visualization design differed in how continuously they presented data. Bar graphs and group-flavoured text descriptions illustrated a clear upward trend in the data, similar to line graphs, but they divided the data into two groups, one group for when the x---dimension variable is of smaller values and one for when the x---dimension variable is of larger values. Scatter plots, on the other hand, depicts a less clear upward trend, but it delivers a continuity similar to line graphs without grouping the data points based on one dimension \textcolor{red}{note:(experiment 4 will talk about aggregated vs discretized values). }

How much effect does grouping variables have on perceived causality in visualized data? Experiment 3 expands the comparison done in experiment 2, adding a scatter plot which, similar to a bar graph with two bars, divides the x---variable dimension into two groups, a bar graph that more finely divides the data into seven groups to look more similar to the line graph, and a text description that, instead of depicting variable relations by grouping them, describes a continuous trend correlating the two variables. We visualized the three new visualization designs, in comparison to those used in Experiment 2, in \textcolor{red}{Figure \ref{fig:7visualizationdesigns}}.

A omnibus power analysis, based on pilot effect sizes, suggested a target sample of 55 participants in a within-subject design comparing seven perceived causality rating, each for one of the seven visualization designs, would be sufficient to detect an overall effect of visualization designs. We iteratively sampled MTurk participants and excluded participants who failed the attention checks or provided wrong answers to the graph comprehension questions until we had 55 participants. 

\subsection{Design and Procedure}
\textcolor{red}{Hey I have a comment!}
Since the quantitative and qualitative questions in Experiment 1 and 2 both yielded similar results, we excluded the text response question in Experiment 3. Additionally, we numerically labelled the x and y---axis of the visualizations in this experiment, and counterbalanced the axis label with four sets of values. This means each participant in Experiment 3 viewed the seven visualization designs in random order, each presented with one of four sets possible axis labels, and only rated how much they agree with a correlation statement and a causation statement on a slider scale.

\subsection{Results}
Mixed-effect linear model revealed that visualization design is a significant predictor to perceived causality (\begin{math}\chi^{2}=115.46\end{math},$p$<0.001). Referring to \textcolor{red}{Figure \ref{fig:Exp3ab_Exp4_consolidated}}, post-hoc comparisons with Tukey adjustments revealed that line graph and bar graph with 7 bars perceived to be the most causal. Scatter plot with 100 points was perceived to be the least causal. Text description of a trend, bar graph with 2 bars, scatter plot with 2 scatter points and grouping text description were in the middle. 

% Tukey groupings for reference
line            a
7bar            ab 
trend           db*
2bar            d
2scatter        d
group           de.
manyscatter     e

\subsection{Modification}
We observed that visualization designs that depict a clear trend to elicit more causal response from participants, compared to visualization designs that makes the trend less clear. Visualization designs grouping variables into only two groups were perceived less causal than designs that created more groups and thus made the data seem more continuous and the upward trend more obvious. However, we also suspect the amount of available data in different visualization designs might have been misleading to participants. For example, the scatter plot with only two scatter points could have been perceived less correlated and less causal had participants interpreted the two scatter points as data collected from only two respondent,instead of data aggregated from fifty people, which is evident in the 100 scatter points design. We address this problem in a follow-up Experiment 3b where we explicitly tell the participants about the sample size included in the visualizations.

\subsection{Experiment 3b}

\jessica{I'm not sure why we are reporting on the no sample size version above if its flawed. Why not just report on it with sample size? Also, not sure we need either experiment 3 bc it is still confounded with aggregation.}
In Experiment 3b, we added a short description of the data before each visualization. For example, the text that accompanies the scatter plot with two points is as follows:
\vspace{3pt}
\noindent\textit{The following graph gives you information regarding factor Q and W, based on a survey from 100 participants.Each of the two points in the graph summarizes the data from approximately half of the participants.}

Compared to the text with the scatter plot with fifty points:
\vspace{3pt}
\noindent\textit{The following graph gives you information regarding factor N and R, based on a survey from 100 participants. Each of the points in the graph shows the data for a single participant.}

\subsection{Experiment 3b Results}
Despite the modification, Experiment 3 yielded very similar results compared to Experiment 3, as shown in the right column in \textcolor{red}{Figure \ref{fig:Exp3ab_Exp4_consolidated}}. Mixed-effect linear model again revealed that visualization design is a significant predictor to perceived causality (\begin{math}\chi^{2}=78.69\end{math},$p$<0.001). Post-hoc comparisons with Tukey adjustments revealed similar comparison groups between Experiment 3 and Experiment 3b such that line graph and bar graph with 7 bars perceived to be the most causal and satter plot with 100 points was perceived to be the least causal.

% Tukey groupings for reference
line            a
7bar            a
trend           ad
2bar            bd
2scatter        bc
group           bc
manyscatter     c

\subsection{Discussion}
We replicated the findings in Experiment 2 revealing that line and bars graphs and plain text invites more false causality assumptions than scatter plots. By comparing bar graphs with only 2 bars and 7 bars, as well as comparing the group-text and trend-text conditions, we see evidence supporting causality perception to be closely associated with how continuous the data is and how clear the trend is depicted. Furthermore, by comparing the scatter plots with 2 scatter points and 100 scatter points, we found that discretizing data by showing every individual points effectively reduce the perception of causality in data. 

Why are graphs and line graphs perceived more casual than scatter plots? Not only they present different information, these visualization designs fundamentally manipulate the data differently. Line graphs show data in a continuous way, but bar graphs and scatter plots less so. Line graphs and bar graphs aggregate the data, while scatter plot shows discretized data points. Experiment 3 addressed that the more continuous the data to depict a more clear trend, the more causal the data is perceived. But it doesn't address whether aggregating or discretizing data is \textit{causing} it. 





 
